Fuzzing: On Benchmarking Outcome as a Function of Benchmark Properties

Characteristics of a benchmarking setup clearly can have some impact on the benchmark outcome. In this paper, we explore two methodologies to quantify the impact of the specific properties on the benchmarking outcome. Our first methodology is the controlled experiment to identify a causal relationship between a single property in isolation and the benchmarking outcome. However, manipulating one property exactly may not always be practical or possible. Hence, our second methodology is randomization and non-parametric regression to identify the strength of the relationship between arbitrary benchmark properties (i.e., covariates) and outcome. Together, these two fundamental aspects of experimental design, control and randomization, can provide a comprehensive picture of the impact of various properties of the current benchmark on the fuzzer ranking. These analyses can be used to guide fuzzer developers towards areas of improvement in their tools and allow researchers to make more nuanced claims about fuzzer effectiveness. We instantiate each approach on a subset of properties suspected of impacting the relative effectiveness of fuzzers and quantify the effects of these properties on the evaluation outcome. In doing so, we identify multiple novel properties which can have statistically significant effect on the relative effectiveness of fuzzers.

==> assets/np-boot/afl_mr_val.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 15:19:16 2022
\begin{tabular}{@{ }r@{ }r@{ }r@{ }r}
  \hline
term & estimate & low & high \\ 
  \hline
initial\_coverage & 0.78 & 0.71 & 0.86 \\ 
  mean\_exec\_ns & 0.01 & -0.06 & 0.08 \\ 
  mean\_size\_bytes & -0.01 & -0.06 & 0.04 \\ 
   \hline
\end{tabular}
R2: 0.849977212524905


==> assets/np-boot/aflplusplus_mr_val.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 15:19:16 2022
\begin{tabular}{@{ }r@{ }r@{ }r@{ }r}
  \hline
term & estimate & low & high \\ 
  \hline
initial\_coverage & 0.47 & 0.38 & 0.57 \\ 
  mean\_exec\_ns & 0.03 & -0.04 & 0.11 \\ 
  mean\_size\_bytes & 0.01 & -0.03 & 0.06 \\ 
   \hline
\end{tabular}
R2: 0.657274618319239


==> assets/np-boot/entropic_mr_val.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 15:19:16 2022
\begin{tabular}{@{ }r@{ }r@{ }r@{ }r}
  \hline
term & estimate & low & high \\ 
  \hline
initial\_coverage & 0.56 & 0.47 & 0.66 \\ 
  mean\_exec\_ns & 0.00 & -0.06 & 0.08 \\ 
  mean\_size\_bytes & -0.01 & -0.06 & 0.04 \\ 
   \hline
\end{tabular}
R2: 0.706849247049852


==> assets/np-boot/libfuzzer_mr_val.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 15:19:16 2022
\begin{tabular}{@{ }r@{ }r@{ }r@{ }r}
  \hline
term & estimate & $<$2.5\% & high \\ 
  \hline
initial\_coverage & 0.62 & 0.54 & 0.70 \\ 
  mean\_exec\_ns & -0.02 & -0.08 & 0.04 \\ 
  mean\_size\_bytes & -0.06 & -0.12 & -0.01 \\ 
   \hline 
\end{tabular} 
R2: 0.811738407782086


==> assets/polr-e1/afl.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Thu Aug 25 10:06:53 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & 3.97 & 0.00 & 52.83 \\ 
  mean\_size\_bytes & -3.28 & 0.01 & 0.04 \\ 
  mean\_exec\_ns & 0.13 & 0.91 & 1.14 \\ 
   \hline
\end{tabular}
BW (0.05): 4/7, HLp: 0.20


==> assets/polr-e1/afl_complex.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Thu Aug 25 10:06:55 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & 3.11 & 0.01 & 22.42 \\ 
  mean\_size\_bytes & -2.99 & 0.01 & 0.05 \\ 
  mean\_exec\_ns & -0.11 & 0.93 & 0.90 \\ 
  corpuse1v0-libfuzzer:initial\_coverage & 2.41 & 0.25 & 11.09 \\ 
   \hline
\end{tabular}
BW (0.05): 6/8, HLp: 0.17


==> assets/polr-e1/aflplusplus.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Thu Aug 25 10:06:53 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & 2.15 & 0.03 & 8.57 \\ 
  mean\_size\_bytes & -2.58 & 0.02 & 0.08 \\ 
  mean\_exec\_ns & -0.80 & 0.46 & 0.45 \\ 
   \hline
\end{tabular}
BW (0.05): 4/7, HLp: 0.71


==> assets/polr-e1/aflplusplus_complex.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Thu Aug 25 10:06:55 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & 2.76 & 0.15 & 15.82 \\ 
  mean\_size\_bytes & -2.67 & 0.03 & 0.07 \\ 
  mean\_exec\_ns & -0.81 & 0.47 & 0.44 \\ 
  benchmarksqlite3\_ossfuzz:initial\_coverage & -2.88 & 0.47 & 0.06 \\ 
  benchmarkzlib\_zlib\_uncompress\_fuzzer:initial\_coverage & -1.32 & 0.59 & 0.27 \\ 
  corpuse1v0-libfuzzer:initial\_coverage & 0.32 & 0.90 & 1.38 \\ 
   \hline
\end{tabular}
BW (0.05): 7/10, HLp: 0.22


==> assets/polr-e1/entropic.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Thu Aug 25 10:06:53 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & -2.50 & 0.00 & 0.08 \\ 
  mean\_exec\_ns & 1.68 & 0.08 & 5.38 \\ 
  mean\_size\_bytes & 3.09 & 0.00 & 21.94 \\ 
   \hline
\end{tabular}
BW (0.05): 5/7, HLp: 0.08


==> assets/polr-e1/entropic_complex.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Thu Aug 25 10:06:54 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & -4.27 & 0.07 & 0.01 \\ 
  mean\_exec\_ns & 1.99 & 0.16 & 7.31 \\ 
  mean\_size\_bytes & 1.33 & 0.43 & 3.77 \\ 
  corpuse1v0-libfuzzer:initial\_coverage & 1.31 & 0.65 & 3.69 \\ 
  benchmarksqlite3\_ossfuzz:initial\_coverage & 1.58 & 0.45 & 4.84 \\ 
  benchmarkzlib\_zlib\_uncompress\_fuzzer:initial\_coverage & 2.84 & 0.28 & 17.13 \\ 
  corpuse1v0-libfuzzer:mean\_size\_bytes & 3.62 & 0.26 & 37.19 \\ 
  corpuse1v0-libfuzzer:mean\_exec\_ns & -1.04 & 0.62 & 0.35 \\ 
  initial\_coverage:mean\_size\_bytes & -4.68 & 0.40 & 0.01 \\ 
  initial\_coverage:mean\_exec\_ns & 2.18 & 0.58 & 8.88 \\ 
   \hline
\end{tabular}
BW (0.05): 12/14, HLp: 0.06


==> assets/polr-e1/libfuzzer.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Thu Aug 25 10:06:52 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & -2.79 & 0.02 & 0.06 \\ 
  mean\_exec\_ns & -1.17 & 0.37 & 0.31 \\ 
  mean\_size\_bytes & 1.60 & 0.22 & 4.96 \\ 
   \hline
\end{tabular}
BW (0.05): 5/7, HLp: 0.00


==> assets/polr-e2/afl.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 14:29:57 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & 0.18 & 0.01 & 1.20 \\ 
  mean\_size\_bytes & 0.09 & 0.14 & 1.09 \\ 
  mean\_exec\_ns & 0.09 & 0.17 & 1.09 \\ 
   \hline
\end{tabular}
BW (0.05): 14/14, HLp: 0.05


==> assets/polr-e2/afl_complex.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 14:29:58 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & -0.10 & 0.55 & 0.91 \\ 
  mean\_size\_bytes & 0.10 & 0.13 & 1.10 \\ 
  mean\_exec\_ns & 0.09 & 0.22 & 1.09 \\ 
  benchmarkharfbuzz-1.3.2:initial\_coverage & -0.08 & 0.74 & 0.93 \\ 
  benchmarklibjpeg-turbo-07-2017:initial\_coverage & 0.47 & 0.11 & 1.60 \\ 
  benchmarklibpcap\_fuzz\_both:initial\_coverage & 1.08 & 0.01 & 2.94 \\ 
  benchmarklibpng-1.2.56:initial\_coverage & 0.34 & 1.00 & 1.41 \\ 
  benchmarklibxslt\_xpath:initial\_coverage & 0.20 & 0.41 & 1.23 \\ 
  benchmarkmbedtls\_fuzz\_dtlsclient:initial\_coverage & 1.66 & 0.18 & 5.24 \\ 
  benchmarksqlite3\_ossfuzz:initial\_coverage & 0.36 & 0.13 & 1.43 \\ 
  benchmarkvorbis-2017-12-11:initial\_coverage & 0.55 & 0.02 & 1.73 \\ 
  benchmarkwoff2-2016-05-06:initial\_coverage & 0.20 & 0.54 & 1.22 \\ 
  benchmarkzlib\_zlib\_uncompress\_fuzzer:initial\_coverage & 0.59 & 0.39 & 1.81 \\ 
   \hline
\end{tabular}
BW (0.05): NA/NA, HLp: 0.22


==> assets/polr-e2/aflplusplus.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 14:29:56 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & 0.12 & 0.09 & 1.13 \\ 
  mean\_size\_bytes & 0.09 & 0.18 & 1.09 \\ 
  mean\_exec\_ns & 0.19 & 0.01 & 1.21 \\ 
   \hline
\end{tabular}
BW (0.05): 14/14, HLp: 1.00


==> assets/polr-e2/entropic.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 14:29:54 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & 0.02 & 0.73 & 1.02 \\ 
  mean\_size\_bytes & -0.05 & 0.36 & 0.95 \\ 
  mean\_exec\_ns & -0.08 & 0.20 & 0.93 \\ 
   \hline
\end{tabular}
BW (0.05): 14/14, HLp: 0.00


==> assets/polr-e2/entropic_complex.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 14:29:59 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & 0.11 & 0.48 & 1.12 \\ 
  mean\_size\_bytes & -0.04 & 0.47 & 0.96 \\ 
  mean\_exec\_ns & -0.01 & 0.91 & 0.99 \\ 
  benchmarkharfbuzz-1.3.2:initial\_coverage & 0.10 & 0.65 & 1.11 \\ 
  benchmarklibjpeg-turbo-07-2017:initial\_coverage & -0.66 & 0.03 & 0.52 \\ 
  benchmarklibpcap\_fuzz\_both:initial\_coverage & 0.94 & 0.02 & 2.57 \\ 
  benchmarklibpng-1.2.56:initial\_coverage & -0.22 & 0.34 & 0.80 \\ 
  benchmarklibxslt\_xpath:initial\_coverage & -0.03 & 0.91 & 0.97 \\ 
  benchmarkmbedtls\_fuzz\_dtlsclient:initial\_coverage & 0.03 & 0.87 & 1.03 \\ 
  benchmarksqlite3\_ossfuzz:initial\_coverage & -0.09 & 0.70 & 0.91 \\ 
  benchmarkvorbis-2017-12-11:initial\_coverage & -0.15 & 0.53 & 0.86 \\ 
  benchmarkwoff2-2016-05-06:initial\_coverage & -0.76 & 0.22 & 0.47 \\ 
  benchmarkzlib\_zlib\_uncompress\_fuzzer:initial\_coverage & -0.15 & 0.64 & 0.86 \\ 
   \hline
\end{tabular}
BW (0.05): NA/NA, HLp: 0.00


==> assets/polr-e2/libfuzzer.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 14:29:51 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & -0.17 & 0.00 & 0.85 \\ 
  mean\_size\_bytes & -0.13 & 0.03 & 0.88 \\ 
  mean\_exec\_ns & -0.16 & 0.01 & 0.85 \\ 
   \hline
\end{tabular}
BW (0.05): 13/14, HLp: 0.95


==> assets/rank-boot/afl_mr.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sun Aug 28 00:51:55 2022
\begin{tabular}{@{ }r@{ }r@{ }r@{ }r}
  \hline
term & estimate & conf.low & conf.high \\ 
  \hline
initial\_coverage & 0.92 & 0.86 & 0.95 \\ 
  mean\_exec\_ns & -0.03 & -0.09 & 0.01 \\ 
  mean\_size\_bytes & 0.01 & -0.04 & 0.06 \\ 
   \hline
\end{tabular}
R2: 0.85


==> assets/rank-boot/aflplusplus_mr.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sun Aug 28 00:51:55 2022
\begin{tabular}{@{ }r@{ }r@{ }r@{ }r}
  \hline
term & estimate & conf.low & conf.high \\ 
  \hline
initial\_coverage & 0.77 & 0.68 & 0.85 \\ 
  mean\_exec\_ns & 0.08 & 0.00 & 0.17 \\ 
  mean\_size\_bytes & -0.06 & -0.15 & 0.02 \\ 
   \hline
\end{tabular}
R2: 0.56


==> assets/rank-boot/entropic_mr.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sun Aug 28 00:51:55 2022
\begin{tabular}{@{ }r@{ }r@{ }r@{ }r}
  \hline
term & estimate & conf.low & conf.high \\ 
  \hline
initial\_coverage & 0.79 & 0.70 & 0.87 \\ 
  mean\_exec\_ns & 0.03 & -0.05 & 0.12 \\ 
  mean\_size\_bytes & -0.06 & -0.14 & 0.01 \\ 
   \hline
\end{tabular}
R2: 0.60


==> assets/rank-boot/libfuzzer_mr.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sun Aug 28 00:51:55 2022
\begin{tabular}{@{ }r@{ }r@{ }r@{ }r}
  \hline
term & estimate & conf.low & conf.high \\ 
  \hline
initial\_coverage & 0.77 & 0.68 & 0.84 \\ 
  mean\_exec\_ns & -0.03 & -0.10 & 0.05 \\ 
  mean\_size\_bytes & -0.10 & -0.19 & -0.02 \\ 
   \hline
\end{tabular}
R2: 0.55


==> assets/rank-boot/none_unified_model.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sun Aug 28 00:51:43 2022
\begin{tabular}{@{ }r@{ }r@{ }r@{ }r}
  \hline
term & estimate & conf.low & conf.high \\ 
  \hline
(Intercept) & 1.34 & 0.27 & 2.45 \\ 
  fuzzeraflplusplus & 1.28 & -0.58 & 3.30 \\ 
  fuzzerentropic & 1.69 & -0.05 & 3.54 \\ 
  fuzzerlibfuzzer & 3.16 & 1.35 & 5.15 \\ 
  initial\_coverage & 0.92 & 0.87 & 0.96 \\ 
  mean\_size\_bytes & 0.01 & -0.04 & 0.07 \\ 
  mean\_exec\_ns & -0.03 & -0.08 & 0.01 \\ 
  fuzzeraflplusplus:initial\_coverage & -0.14 & -0.24 & -0.06 \\ 
  fuzzerentropic:initial\_coverage & -0.12 & -0.21 & -0.04 \\ 
  fuzzerlibfuzzer:initial\_coverage & -0.15 & -0.24 & -0.06 \\ 
  fuzzeraflplusplus:mean\_size\_bytes & -0.07 & -0.17 & 0.03 \\ 
  fuzzerentropic:mean\_size\_bytes & -0.07 & -0.16 & 0.01 \\ 
  fuzzerlibfuzzer:mean\_size\_bytes & -0.12 & -0.21 & -0.02 \\ 
  fuzzeraflplusplus:mean\_exec\_ns & 0.11 & 0.02 & 0.22 \\ 
  fuzzerentropic:mean\_exec\_ns & 0.06 & -0.03 & 0.15 \\ 
  fuzzerlibfuzzer:mean\_exec\_ns & 0.01 & -0.09 & 0.10 \\ 
   \hline
\end{tabular}
R2: 0.64


==> assets/simple-linreg/afl_fuzzer_rank_multi.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 13:11:36 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{ }r}
  \hline
 & term & estimate & conf.low & conf.high \\ 
  \hline
1 & initial\_coverage & 0.01 & 1.58 & -0.76 \\ 
  2 & mean\_exec\_ns & 0.00 & 1.58 & -0.76 \\ 
  3 & mean\_size\_bytes & 0.00 & 1.58 & -0.76 \\ 
   \hline
\end{tabular}
R2: 0.422896546918477


==> assets/simple-linreg/afl_fuzzer_rank_single.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 13:30:54 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{ }r}
  \hline
 & term & estimate & conf.low & conf.high \\ 
  \hline
1 & corpus\_size & 0.00678448315469405 & 1.16926770386123 & -0.0111004374717161 \\ 
  2 & initial\_coverage & 0.0120355731225296 & 1.2683572190542 & 0.00171370358891954 \\ 
  3 & mean\_exec\_ns & 0.00294466403162052 & 1.39743738294843 & -0.00629636463566887 \\ 
  4 & mean\_size\_bytes & 0.00634387351778652 & 1.36557820051692 & -0.00215314460536728 \\ 
  5 & q100\_exec\_ns & 0.00776679841897231 & 1.35484051758155 & -0.000236900985149618 \\ 
  6 & q100\_mean\_size\_bytes & 0.00881693426406274 & 1.20491224761812 & -0.00948532416901133 \\ 
   \hline
\end{tabular}
R2: 0.0152819217143326


==> assets/simple-linreg/afl_value_rank_multi.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 13:30:54 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{ }r}
  \hline
 & term & estimate & conf.low & conf.high \\ 
  \hline
1 & initial\_coverage & -31.99 & 764.72 & -145.24 \\ 
  2 & mean\_exec\_ns & 2.11 & 764.72 & -145.24 \\ 
  3 & mean\_size\_bytes & -0.04 & 764.72 & -145.24 \\ 
   \hline
\end{tabular}
R2: 0.730616729568323


==> assets/simple-linreg/afl_value_rank_single.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 13:30:54 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{ }r}
  \hline
 & term & estimate & conf.low & conf.high \\ 
  \hline
1 & initial\_coverage & -46.470909090909 & 1262.63205612386 & -60.1857021506469 \\ 
  2 & mean\_exec\_ns & 2.48474308300399 & 634.735551069683 & -12.3463771344151 \\ 
  3 & mean\_size\_bytes & -12.8914624505928 & 828.081897767108 & -27.6425349159677 \\ 
  4 & corpus\_size & -44.4347653929915 & 1235.59710041939 & -58.2632431149264 \\ 
  5 & q100\_mean\_size\_bytes & -31.9507575757575 & 1069.94408361275 & -46.498974322198 \\ 
  6 & q100\_exec\_ns & -27.6716205533597 & 1017.17559142944 & -42.1188360992245 \\ 
   \hline
\end{tabular}
R2: 0.14522806652422


==> assets/simple-linreg/aflplusplus_fuzzer_rank_multi.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 13:11:36 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{ }r}
  \hline
 & term & estimate & conf.low & conf.high \\ 
  \hline
1 & initial\_coverage & 0.01 & 3.42 & -0.30 \\ 
  2 & mean\_exec\_ns & 0.01 & 3.42 & -0.30 \\ 
  3 & mean\_size\_bytes & 0.00 & 3.42 & -0.30 \\ 
   \hline
\end{tabular}
R2: 0.49530837752004


==> assets/simple-linreg/aflplusplus_fuzzer_rank_single.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 13:30:54 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{ }r}
  \hline
 & term & estimate & conf.low & conf.high \\ 
  \hline
1 & corpus\_size & -0.00185573299984379 & 3.28091706561629 & -0.0197845043676307 \\ 
  2 & initial\_coverage & 0.00604743083003948 & 3.30650736143082 & -0.00458969969181607 \\ 
  3 & mean\_exec\_ns & 0.0141897233201581 & 3.1911166805284 & 0.00259994951066913 \\ 
  4 & mean\_size\_bytes & 0.00667984189723312 & 3.30013865048989 & -0.00384976110592611 \\ 
  5 & q100\_exec\_ns & 0.00628458498023705 & 3.28690846842361 & -0.00551671566051804 \\ 
  6 & q100\_mean\_size\_bytes & -0.000424389240578659 & 3.21775152428166 & -0.022462122822047 \\ 
   \hline
\end{tabular}
R2: 0.00115407751864464


==> assets/simple-linreg/aflplusplus_value_rank_multi.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 13:11:36 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{ }r}
  \hline
 & term & estimate & conf.low & conf.high \\ 
  \hline
1 & initial\_coverage1 & -33.81 & 1116.07 & -149.65 \\ 
  2 & mean\_exec\_ns1 & 4.78 & 1116.07 & -149.65 \\ 
  3 & mean\_size\_bytes1 & -0.88 & 1116.07 & -149.65 \\ 
   \hline
\end{tabular}
R2: 0.801567690124283


==> assets/simple-linreg/aflplusplus_value_rank_single.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 13:30:54 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{ }r}
  \hline
 & term & estimate & conf.low & conf.high \\ 
  \hline
1 & initial\_coverage & -81.3335968379445 & 2154.10630755886 & -110.226124801335 \\ 
  2 & mean\_exec\_ns & -3.19841897233195 & 1153.91630858878 & -33.735623625924 \\ 
  3 & mean\_size\_bytes & -23.8307509881422 & 1413.75552007714 & -54.2325295622119 \\ 
  4 & corpus\_size & -77.7998020194021 & 2107.5592003991 & -106.864589429273 \\ 
  5 & q100\_mean\_size\_bytes & -58.2250733137829 & 1848.33202998178 & -88.4064892936074 \\ 
  6 & q100\_exec\_ns & -53.4298023715415 & 1791.7705396125 & -83.2698165606683 \\ 
   \hline
\end{tabular}
R2: 0.104960860553637


==> assets/simple-linreg/entropic_fuzzer_rank_multi.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 13:11:36 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{ }r}
  \hline
 & term & estimate & conf.low & conf.high \\ 
  \hline
1 & initial\_coverage & 0.01 & 2.65 & -0.38 \\ 
  2 & mean\_exec\_ns & -0.00 & 2.65 & -0.38 \\ 
  3 & mean\_size\_bytes & -0.00 & 2.65 & -0.38 \\ 
   \hline
\end{tabular}
R2: 0.271490006335083


==> assets/simple-linreg/entropic_fuzzer_rank_single.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 13:30:54 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{ }r}
  \hline
 & term & estimate & conf.low & conf.high \\ 
  \hline
1 & corpus\_size & 0.00301556746829569 & 2.91397162957991 & -0.0118726610430551 \\ 
  2 & initial\_coverage & 0.00474308300395251 & 2.9429294751548 & -0.00491025126550001 \\ 
  3 & mean\_exec\_ns & -0.00430830039525695 & 3.02517072019389 & -0.0161242574867822 \\ 
  4 & mean\_size\_bytes & -0.00193675889328067 & 3.02272514595056 & -0.0118492038913292 \\ 
  5 & q100\_exec\_ns & -0.000671936758893293 & 2.97842986868564 & -0.0125779165214082 \\ 
  6 & q100\_mean\_size\_bytes & 0.00109474124351742 & 2.88490467539152 & -0.0162420954253767 \\ 
   \hline
\end{tabular}
R2: 0.00440495352776566


==> assets/simple-linreg/entropic_value_rank_multi.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 13:11:36 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{ }r}
  \hline
 & term & estimate & conf.low & conf.high \\ 
  \hline
1 & initial\_coverage2 & -34.64 & 896.67 & -46.37 \\ 
  2 & mean\_exec\_ns2 & 3.49 & 896.67 & -46.37 \\ 
  3 & mean\_size\_bytes2 & -0.76 & 896.67 & -46.37 \\ 
   \hline
\end{tabular}
R2: 0.80593665533194


==> assets/simple-linreg/entropic_value_rank_single.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 13:30:54 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{ }r}
  \hline
 & term & estimate & conf.low & conf.high \\ 
  \hline
1 & initial\_coverage & -55.1748616600789 & 1614.20863604231 & -73.9585149028072 \\ 
  2 & mean\_exec\_ns & 3.43343873517792 & 865.047085625359 & -16.509018798469 \\ 
  3 & mean\_size\_bytes & -16.5009486166007 & 1115.6112975966 & -36.3465204274902 \\ 
  4 & corpus\_size & -52.7161354187289 & 1581.7739356529 & -71.6227540330801 \\ 
  5 & q100\_mean\_size\_bytes & -39.2102883675464 & 1402.84158613413 & -58.8888527140806 \\ 
  6 & q100\_exec\_ns & -33.3641106719367 & 1330.91649591373 & -52.8936512320332 \\ 
   \hline
\end{tabular}
R2: 0.113227306319244


==> assets/simple-linreg/libfuzzer_fuzzer_rank_multi.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 13:11:36 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{ }r}
  \hline
 & term & estimate & conf.low & conf.high \\ 
  \hline
1 & initial\_coverage & -0.02 & 1.13 & 0.19 \\ 
  2 & mean\_exec\_ns & -0.01 & 1.13 & 0.19 \\ 
  3 & mean\_size\_bytes & -0.00 & 1.13 & 0.19 \\ 
   \hline
\end{tabular}
R2: 0.504231487411256


==> assets/simple-linreg/libfuzzer_fuzzer_rank_single.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 13:30:54 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{ }r}
  \hline
 & term & estimate & conf.low & conf.high \\ 
  \hline
1 & corpus\_size & -0.00794431762314587 & 1.60618334277876 & -0.0308647216040689 \\ 
  2 & initial\_coverage & -0.0181620553359684 & 1.81474343549963 & -0.0301821881243139 \\ 
  3 & mean\_exec\_ns & -0.0128260869565217 & 1.74228768767671 & -0.025249065842926 \\ 
  4 & mean\_size\_bytes & -0.0110869565217392 & 1.73156622244057 & -0.0227388594683289 \\ 
  5 & q100\_exec\_ns & -0.0133794466403162 & 1.75043530718148 & -0.0257162998256926 \\ 
  6 & q100\_mean\_size\_bytes & -0.00948728626700149 & 1.51948323315816 & -0.0358843925121107 \\ 
   \hline
\end{tabular}
R2: 0.012790413459396


==> assets/simple-linreg/libfuzzer_value_rank_multi.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 13:11:37 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{ }r}
  \hline
 & term & estimate & conf.low & conf.high \\ 
  \hline
1 & initial\_coverage3 & -35.29 & 681.66 & 31.38 \\ 
  2 & mean\_exec\_ns3 & -0.50 & 681.66 & 31.38 \\ 
  3 & mean\_size\_bytes3 & -3.29 & 681.66 & 31.38 \\ 
   \hline
\end{tabular}
R2: 0.789962788888212


==> assets/simple-linreg/libfuzzer_value_rank_single.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 13:30:54 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{ }r}
  \hline
 & term & estimate & conf.low & conf.high \\ 
  \hline
1 & initial\_coverage & -48.0254150197627 & 1235.08982858341 & -60.2408281242803 \\ 
  2 & mean\_exec\_ns & -3.23916996047425 & 656.408398182281 & -16.774043907146 \\ 
  3 & mean\_size\_bytes & -20.7213833992094 & 878.236259276491 & -34.0252919409612 \\ 
  4 & corpus\_size & -44.8618095426648 & 1192.86841237456 & -57.2671174757616 \\ 
  5 & q100\_mean\_size\_bytes & -36.948761811665 & 1086.21392805301 & -49.9384090899195 \\ 
  6 & q100\_exec\_ns & -30.2678656126482 & 1001.47578090201 & -43.2982365584368 \\ 
   \hline
\end{tabular}
R2: 0.186158283626948


==> assets/simple-linreg/none_value_rank_single_no_fuzzer.tex <==
% latex table generated in R 4.0.4 by xtable 1.8-4 package
% Sat Aug 27 13:30:54 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{ }r}
  \hline
 & term & estimate & conf.low & conf.high \\ 
  \hline
1 & initial\_coverage & -34.5621739130435 & 936.963277779792 & -36.2113031095692 \\ 
  2 & mean\_exec\_ns & 5.77467391304346 & 418.616312207367 & 3.13620506523563 \\ 
  3 & mean\_size\_bytes & -11.230652173913 & 632.112083327173 & -13.804090915949 \\ 
  4 & corpus\_size & -31.4225202930113 & 894.597255736301 & -33.2904185322767 \\ 
  5 & q100\_mean\_size\_bytes & -22.4966397849463 & 776.465608070971 & -24.8312361176554 \\ 
  6 & q100\_exec\_ns & -18.619347826087 & 726.780023597762 & -21.0311731107977 \\ 
   \hline
\end{tabular}
R2: 0.616052735700202


==> nsections/figures/linear.corpus.tex <==
 & \textbf{\#Seeds} & \textbf{Initial Coverage} & \textbf{Mean Exec Time} & \textbf{Mean Seed Size}\\
afl & 3.3+0.06x (0.17) &3.3+0.07x (0.21) &3.4+0.06x (0.05) &3.3+0.07x (0.12)\\
aflplusplus & 1.4+0.07x (0.02) &1.4+0.07x (0.06) &1.2+0.08x (0.31) &1.3+0.07x (0.18)\\
entropic & 1.8+0.07x (0.04) &1.8+0.07x (0.05) &1.9+0.08x (0.04) &1.9+0.07x (0.02)\\
libfuzzer & 3.4+0.07x (0.32) &3.5+0.08x (0.31) &3.4+0.08x (0.27) &3.4+0.08x (0.23)\\


==> nsections/figures/linear.program.tex <==
 & \textbf{Program Size} & \textbf{\#Equalities} & \textbf{total_indir} & \textbf{\#Inqualities} & \textbf{\#Shared Libraries}\\
afl & 3.1+0.25x (0.22) &3.2+0.27x (0.10) &3.1+0.25x (0.22) &3.1+0.25x (0.23) &3.3+0.28x (0.06)\\
aflplusplus & 0.8+0.24x (0.51) &0.9+0.26x (0.43) &0.8+0.24x (0.51) &0.9+0.26x (0.43) &1.0+0.30x (0.26)\\
entropic & 2.0+0.23x (0.08) &2.0+0.23x (0.03) &2.0+0.23x (0.08) &2.0+0.23x (0.03) &2.0+0.24x (0.02)\\
libfuzzer & 4.1+0.27x (0.57) &4.0+0.31x (0.45) &4.1+0.27x (0.57) &4.1+0.26x (0.60) &3.8+0.36x (0.26)\\


==> nsections/figures/linear.regression.tex <==
 & \multicolumn{4}{c}{\emph{Corpus}} & \multicolumn{4}{c}{\emph{Program}}\\
 & \emph{\#Seeds} & \emph{Initial Coverage} & \emph{Mean Exec Time} & \emph{Mean Seed Size} & \emph{Program Size} & \emph{\#Equalities} & \emph{\#Inqualities} & \emph{\#Shared Libraries}\\\hline
\emph{AFL} & \textbf{\textcolor{darkred}{3.3 + 0.008x}} &\textbf{\textcolor{darkred}{3.3 + 0.012x}} &\textcolor{darkred}{3.4 + 0.004x} &\textcolor{darkred}{3.3 + 0.008x} &\textcolor{darkred}{3.1 + 0.058x} &\textcolor{darkred}{3.2 + 0.040x} &\textcolor{darkred}{3.1 + 0.059x} &\textcolor{darkred}{3.3 + 0.030x}\\
\emph{AFL++} & \textcolor{darkred}{1.4 + 0.003x} &\textcolor{darkred}{1.4 + 0.006x} &\textbf{\textcolor{darkred}{1.2 + 0.018x}} &\textbf{\textcolor{darkred}{1.3 + 0.010x}} &\textbf{\textcolor{darkred}{0.8 + 0.109x}} &\textbf{\textcolor{darkred}{0.9 + 0.102x}} &\textbf{\textcolor{darkred}{0.9 + 0.101x}} &\textcolor{darkred}{1.0 + 0.080x}\\
\emph{Entropic} & \textcolor{darkred}{1.8 + 0.005x} &\textcolor{darkred}{1.8 + 0.005x} &\textcolor{darkgreen}{1.9 - 0.006x} &\textcolor{darkgreen}{1.9 - 0.003x} &\textcolor{darkgreen}{2.0 - 0.030x} &\textcolor{darkgreen}{2.0 - 0.018x} &\textcolor{darkgreen}{2.0 - 0.018x} &\textcolor{darkgreen}{2.0 - 0.016x}\\
\emph{Libfuzzer} & \textbf{\textcolor{darkgreen}{3.4 - 0.016x}} &\textbf{\textcolor{darkgreen}{3.5 - 0.018x}} &\textbf{\textcolor{darkgreen}{3.4 - 0.017x}} &\textbf{\textcolor{darkgreen}{3.4 - 0.015x}} &\textbf{\textcolor{darkgreen}{4.1 - 0.137x}} &\textbf{\textcolor{darkgreen}{4.0 - 0.123x}} &\textbf{\textcolor{darkgreen}{4.1 - 0.141x}} &\textcolor{darkgreen}{3.8 - 0.094x}

==> nsections/figures/polr.corpus.afl.old.tex <==
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Mon Aug 22 01:31:37 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & 0.12 & 0.06 & 1.13 \\ 
  corpus\_size & -0.09 & 0.15 & 0.91 \\ 
  mean\_exec\_ns & 0.02 & 0.38 & 1.02 \\ 
  mean\_size\_bytes & 0.01 & 0.63 & 1.01 \\ 
   \hline
\end{tabular}


==> nsections/figures/polr.corpus.afl.tex <==
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Mon Aug 22 01:39:57 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & 0.04 & 0.02 & 1.04 \\ 
  mean\_exec\_ns & 0.02 & 0.21 & 1.02 \\ 
  1$|$2 & -4.84 & 0.00 & 0.01 \\ 
  2$|$2.5 & -1.95 & 0.00 & 0.14 \\ 
   \hline
\end{tabular}


==> nsections/figures/polr.corpus.aflplusplus.old.tex <==
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Mon Aug 22 01:31:37 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & 0.07 & 0.26 & 1.08 \\ 
  corpus\_size & -0.06 & 0.35 & 0.94 \\ 
  mean\_exec\_ns & 0.04 & 0.04 & 1.04 \\ 
  mean\_size\_bytes & 0.01 & 0.57 & 1.01 \\ 
   \hline
\end{tabular}


==> nsections/figures/polr.corpus.aflplusplus.tex <==
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Mon Aug 22 01:39:57 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & 0.02 & 0.27 & 1.02 \\ 
  mean\_exec\_ns & 0.04 & 0.02 & 1.05 \\ 
  1$|$1.5 & 1.50 & 0.00 & 4.50 \\ 
  1.5$|$2 & 1.54 & 0.00 & 4.66 \\ 
   \hline
\end{tabular}


==> nsections/figures/polr.corpus.entropic.old.tex <==
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Mon Aug 22 01:31:37 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & 0.04 & 0.52 & 1.04 \\ 
  corpus\_size & -0.03 & 0.65 & 0.97 \\ 
  mean\_exec\_ns & -0.02 & 0.30 & 0.98 \\ 
  mean\_size\_bytes & -0.02 & 0.37 & 0.98 \\ 
   \hline
\end{tabular}


==> nsections/figures/polr.corpus.entropic.tex <==
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Mon Aug 22 01:39:57 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & 0.01 & 0.65 & 1.01 \\ 
  mean\_exec\_ns & -0.02 & 0.25 & 0.98 \\ 
  1$|$1.5 & -1.24 & 0.00 & 0.29 \\ 
  1.5$|$2 & -1.06 & 0.00 & 0.34 \\ 
   \hline
\end{tabular}


==> nsections/figures/polr.corpus.libfuzzer.old.tex <==
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Mon Aug 22 01:31:37 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & -0.06 & 0.31 & 0.94 \\ 
  corpus\_size & 0.02 & 0.76 & 1.02 \\ 
  mean\_exec\_ns & -0.04 & 0.04 & 0.97 \\ 
  mean\_size\_bytes & -0.01 & 0.42 & 0.99 \\ 
   \hline
\end{tabular}


==> nsections/figures/polr.corpus.libfuzzer.tex <==
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Mon Aug 22 01:39:58 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
initial\_coverage & -0.05 & 0.00 & 0.95 \\ 
  mean\_exec\_ns & -0.04 & 0.02 & 0.96 \\ 
  1$|$1.5 & -4.52 & 0.00 & 0.01 \\ 
  1.5$|$2 & -3.92 & 0.00 & 0.02 \\ 
   \hline
\end{tabular}


==> nsections/figures/polr.program.afl.old.tex <==
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Mon Aug 22 01:32:15 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
total\_shared & 0.26 & 0.03 & 1.29 \\ 
  total\_eq & -0.66 & 0.00 & 0.52 \\ 
  total\_ineq & 0.52 & 0.00 & 1.68 \\ 
  bin\_text\_size & 0.16 & 0.21 & 1.18 \\ 
   \hline
\end{tabular}


==> nsections/figures/polr.program.afl.tex <==
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Mon Aug 22 01:46:00 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
bin\_text\_size & 0.24 & 0.00 & 1.27 \\ 
  1$|$2 & -4.40 & 0.00 & 0.01 \\ 
  2$|$2.5 & -1.53 & 0.00 & 0.22 \\ 
  2.5$|$3 & -1.47 & 0.00 & 0.23 \\ 
   \hline
\end{tabular}


==> nsections/figures/polr.program.aflplusplus.old.tex <==
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Mon Aug 22 01:32:15 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
total\_shared & -0.05 & 0.70 & 0.95 \\ 
  total\_eq & 0.36 & 0.09 & 1.43 \\ 
  total\_ineq & -0.40 & 0.04 & 0.67 \\ 
  bin\_text\_size & 0.49 & 0.00 & 1.64 \\ 
   \hline
\end{tabular}


==> nsections/figures/polr.program.aflplusplus.tex <==
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Mon Aug 22 01:46:00 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
bin\_text\_size & 0.40 & 0.00 & 1.48 \\ 
  1$|$1.5 & 3.32 & 0.00 & 27.53 \\ 
  1.5$|$2 & 3.36 & 0.00 & 28.81 \\ 
  2$|$2.5 & 4.63 & 0.00 & 102.92 \\ 
   \hline
\end{tabular}


==> nsections/figures/polr.program.entropic.old.tex <==
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Mon Aug 22 01:32:15 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
total\_shared & -0.02 & 0.86 & 0.98 \\ 
  total\_eq & -0.08 & 0.68 & 0.92 \\ 
  total\_ineq & 0.43 & 0.01 & 1.54 \\ 
  bin\_text\_size & -0.47 & 0.00 & 0.62 \\ 
   \hline
\end{tabular}


==> nsections/figures/polr.program.entropic.tex <==
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Mon Aug 22 01:46:00 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
bin\_text\_size & -0.14 & 0.00 & 0.87 \\ 
  1$|$1.5 & -1.94 & 0.00 & 0.14 \\ 
  1.5$|$2 & -1.75 & 0.00 & 0.17 \\ 
  2$|$2.5 & 1.34 & 0.00 & 3.80 \\ 
   \hline
\end{tabular}


==> nsections/figures/polr.program.libfuzzer.old.tex <==
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Mon Aug 22 01:32:15 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
total\_shared & -0.10 & 0.35 & 0.90 \\ 
  total\_eq & 0.26 & 0.16 & 1.30 \\ 
  total\_ineq & -0.49 & 0.00 & 0.61 \\ 
  bin\_text\_size & -0.07 & 0.61 & 0.94 \\ 
   \hline
\end{tabular}


==> nsections/figures/polr.program.libfuzzer.tex <==
% latex table generated in R 4.1.0 by xtable 1.8-4 package
% Mon Aug 22 01:46:00 2022
\begin{tabular}{@{}r@{ }r@{ }r@{ }r@{}}
  \hline
 & Value & p\_value & odds\_ratio \\ 
  \hline
bin\_text\_size & -0.35 & 0.00 & 0.70 \\ 
  1$|$1.5 & -5.97 & 0.00 & 0.00 \\ 
  1.5$|$2 & -5.33 & 0.00 & 0.00 \\ 
  2$|$2.5 & -3.98 & 0.00 & 0.02 \\ 
   \hline
\end{tabular}


==> nsections/figures/slr.tex <==
\begin{figure*}[t]
    \centering\footnotesize
    \begin{minipage}{0.32\textwidth}\centering
    \textbf{(a)~Corpus properties.}\\
    \includegraphics[width=\textwidth]{nsections/figures/corpus.rank.pdf}%\\[0.3cm]
    \end{minipage}
    \begin{minipage}{0.32\textwidth}\centering
    \textbf{(b)~Program properties.}\\
    \includegraphics[width=\textwidth]{nsections/figures/program.rank.pdf}
    \end{minipage}%\\[0.3cm] 
    \begin{minipage}{0.325\textwidth}\centering
    \textbf{(c)~Regression Slopes.} (95\%-CIs bootstrapped)\\
    \includegraphics[width=\textwidth]{nsections/figures/coefficients.corpus.pdf}\\[-0.3cm]
    \includegraphics[width=\textwidth]{nsections/figures/coefficients.program.pdf}
    \end{minipage}\vspace{-0.2cm}
    %\begin{minipage}{\textwidth}\centering
    %\begin{tabular}{@{}r@{ }|@{ }r@{ \ }r@{ \ }r@{ \ }r@{ }|@{ }r@{ \ }r@{ \ }r@{ \ }r@{}}
    %\input{nsections/figures/linear.regression}\\
    %\end{tabular}\\[0.2cm]\footnotesize
    %\textbf{(c)~Regression Models} [fuzzer\_rank = intercept + slope * property\_rank; improving ranks in green; stat. signifcant coefficients in bold; $p<0.05$])].
    %\end{minipage}
    \caption{Linear regression between fuzzer ranks and trials ranks w.r.t. benchmark properties.}
    %\vspace{-0.4cm}}
    \label{fig:slr} 
\end{figure*}

==> nsections/figures/spearman-all-corr-heatmap.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{assets/spearman-heatmaps/all-pred.png}
    \label{fig:e2-spearman-all-varcor}
    \caption{Spearman Correlations of Explanatory Variables and Edges Covered}
\end{figure}

==> nsections/motivation.tex <==

\section{Motivation}


% \subsection{Overfitting in Atomistic Evaluations}
% Given a representative benchmark, the assumption of traditional fuzzer evaluation is that the outcome \emph{generalizes} beyond the benchmark itself.
% However, the traditional evaluation on a single benchmark configuration risks overfitting to that configuration which \emph{violates the generality assumption}. In other words, overfitting is a \emph{threat to external validity}.
% If a fuzzer is developed by considering a specific well known bench\-mark, the fuzzer might be unintentionally optimized against the \emph{specific} properties of the benchmark. For instance, about the atomistic evaluation in FuzzBench, we read: %Such \emph{overfitting} violates the objective of sound fuzzer evaluation, i.e., to provide an evaluation of fuzzer performance \emph{in general}. %During repeated experiments, the fuzzer's performance might appear to improve. Yet, in general, the fuzzer's performance may even degrade.

{\small
\result{
``Without knowing what it is about a fuzzer that makes it better on libpng versus libjson, we're really just taking massive leaps where there are hundreds of variables at play. I'd like to see some major changes in the way we evaluate and quantify these results such that we can make predictions about which fuzzers will perform in which ways against certain targets.''
\newline \hspace*{\fill}---\emph{Brandon Falk on FuzzBench \cite{overfitting2}}
}}

% Not conducting a holistic fuzzer evaluation also poses a \emph{threat to internal validity}, i.e., the degree of confidence that our conclusion is not influenced by other factors or variables.
% Consider a recent evaluation of gradient-descent-based fuzzing \cite{angora}.
% The authors implement a gradient-descent-based search together with related changes (e.g., a magic byte extraction) into a baseline fuzzer and run both fuzzers on a well-known benchmark, LAVA-M \cite{gavitt16lava}.
% The results appeared to show gradient-descent as a highly effective fuzzing strategy, but a subsequent investigation found that ``gradient descent contributed little to that success'' relative to magic-byte extraction \cite{overfitting3}.
% A systematic bias in the benchmark created the opportunity for such a misleading outcome: all of the synthetic bugs injected into the LAVA-M benchmark were 32-bit magic byte constraints.
% Our holistic evaluation methodology can mitigate these issues by accounting for properties of the benchmark, such as the constraints present in each subject program.



==> nsections/proportional.tex <==
\newpage
\section{Old. Combined Impact on Benchmarking Outcome}

\subsection{Methodology}
To see the impact of various covariates on the outcome of benchmarking runs, we analyze their effects on the ranking produced by benchmarking tools such as Fuzzbench.
This approach gives us an ordinal outcome for each fuzzer on each of the $k$ trials during an experiment.
To determine the extent to which various covariates impact our ordinal response variable we use Proportional Odds Logistic Regression (POLR).
POLR is an extension of the non-parametric Mann-Whitney U test \cite{harrell_2022_wilcoxon} already widely used in fuzzer benchmarking and advocated by Arcuri and Briand for empirical studies on software programs \cite{harrell1984regression}\cite{arcuri2014hitchhiker}.
It has the advantages, however, of accounting for the effects of covariates, giving  effect size in the form of the model coefficients and predicting outcomes for unseen data.
As with linear regression, the coefficient represents the effect of the corresponding covariate if we were to \emph{hold all other variables constant}.
This representation is in contrast to something like the Vargha-Delaney A-statistic, which cannot account for covariates which may also be influencing the effect size measure.

\subsection{Assumptions}

\subsubsection{Proportional Odds Assumption}
The primary assumption of a POLR model is the Proportional Odds Assumption, which is that no individual variable has an undue influence on a particular level of the outcome variable \cite{mcnulty2021handbookreg}.
This assumption allows the data to be modeled with a single coefficient for each variable across levels, as opposed to a logistic regression for each adjacent category, which would produce several such coefficients.
We do note, however, that POLR models still provide much useful insight when the PO assumption is not met.
Indeed, the Mann-Whitney U test also only has maximum power when the proportional odds assumption is met, yet the assumption is rarely tested \cite{harrell1984regression}.
When the assumption is not met, the coefficients are representative of the net effects across different outcome levels \cite{harrell_2022_not_fatal}.
In our context, having separate coefficients for different ranking levels is not a helpful distinction as we are not concerned with determining the odds of any individual outcome level (e.g. that a fuzzer places 3rd) but rather with changes in the overall ranking of the fuzzer regardless of its position in the rankings.
Still, we found the assumption to generally hold across all of our models according the the Brant-Wald test \cite{brant1990assessing}.
The test compares the coefficients from both the proportional odds model and a generalized ordinal logistic regression model, which allows for different coefficients at each level.
If there is a significant difference in the coefficients, the Brant-Wald test reports so with a \textbf{low p-value}.
Per recommendations in \cite{mcnulty2021handbookreg}, we consider the Proportional Odds assumption to be violated if the Ombnibus test and at least one coefficient tests reports a lower p-value than 0.05.

\subsection{Model Diagnostics}

\subsubsection{Goodness of Fit}

For linear regresion we use $R^{2}$ and adjusted $R^{2}$ to assess model fit.

Fagerland et al \cite{fagerland2016tests} advocate using a combination of three separate tests to assess the goodness of fit of a POLR model; the Pulkstenis-Robinson chi-squared and deviance tests \cite{pulkstenis2004goodness}, the Lipsitz test \cite{lipsitz1996goodness} and the Hosmer-Lemeshow test \cite{fagerland2008multinomial} (\todo{check source on this})
Each of these tests operates similarly, partitioning data into groups and comparing that the observed and fitted values per group with a chi-square test \cite{mcnulty2021handbookreg}.
These tests are designed to detect a variety of issues, such as a potential violation of the proportional odds assumption, a missing interaction term or variable, or an unspecified non-linear relationship.
We find that most of our models do not show signs of poorly fitting the data by these criteria.
Of the models that did indicate significant issues with fitting the data, nearly all issues were resolved by adding additional, per-benchmark interaction terms for some or all independent variables.
However, given that we'd like to understand the effects of various covariates in general rather than their effects on any specific benchmarks, we use the simpler models to obtain coefficients and confidence intervals representing the net effects across benchmarks.


\subsubsection{Variable Selection and Collinearity}
\input{nsections/figures/spearman-all-corr-heatmap}

\todo{Some or most of this may move up to the first section on linear regression, since it's basically all the same}
\todo{need to add correlation with coverage inc to figure}
\todo{actually, this may be better in threats to validity}




\subsubsection{Models}

We perform a single regression per fuzzer against the ranking of that fuzzer's performance per trial.
Our models were each of the form:

$$ranking ~ benchmark + initial coverage + execution time + size$$

\subsection{Results}
For all of our selected explanatory variables we saw significant changes in rankings for at least one fuzzer.
We show the odds-ratios and corresponding confidence intervals for each of our models in Figure \ref{fig:e2-polr-coef-plot}.

\subsubsection{Initial Coverage}
Initial coverage is the strongest predictor among our independent variables for the coverage increase attained by a fuzzer.
However, we see in \ref{fig:e2-polr-tabs} that libfuzzer has 20\% higher odds of a better rank as the initial coverage of the seed corpus increases while AFL has 60\% higher odds of a better rank as the coverage increases.
This reinforces our results in Section (MOTIVATION) that the.
Additionally, AFL is known to have difficulties with extremely low-coverage or empty corpora, so initially having a handful of valid seeds may boost its relative performance.


\subsection{Execution Time}
Execution time also appears to have a substantial impact on relative fuzzer performance.
Looking at Figure \ref{fig:e2-polr-coef-plot}, we see that libfuzzer again performs significantly worse on longer running seeds relative to the other fuzzers while AFL++ performs significantly better on such seedssss

\subsubsection{Seed Size}
The seed size has a far smaller impact on fuzzer rankings in our experiment, but still significantly affects the ranking of libfuzzer, which has 72\% lower odds of a better rank as seed size increases.
This shows that, to at least some extent, fuzzers perform differently on differently sized seeds, even taking into account the effect of initial coverage and execution times.

\subsubsection{Summary}
Overall, we see that each of the predictors that have an influence on overall fuzzer performance in terms of coverage increase also had differing relative performance across fuzzers.
This indicates that picking a seed corpus for fuzzer benchmarking is a fraught task as there are many opportunities for introducing bias.


\input{sections/figures/e2_mr}





==> nsections/setup.tex <==
\section{Experimental Setup}
\todo{Maybe we can accomodate the setup mostly in Section III (Holisitc Fuzzer Benchmarking)}

\subsection{Fuzzers}
\todo{\begin{itemize}
    \item Start this paragraph with a summary and show a table.
\end{itemize}}

We choose two core fuzzer implementations, AFL and Libfuzzer, as many recent works in fuzzing are based on these two implementations.
We also choose two such extensions: AFLplusplus and Entropic\footnote{While AFL++ is technically a fresh implementation, it shares much of the original AFL in it's design}.
Lastly, we take honggfuzz as a separate implementation not based on AFL or libfuzzer which performs strongly in benchmarks.
This gives us three separate core implementations and two derivatives.

\subsection{Seed Sampling and Initial Corpora}

Many current implementations of popular benchmarks like Fuzzbench \cite{metzman2021fuzzbench} use a static set of seeds for each trial.
However, to assess the impact of various initial corpora and benchmarks, we instead sample the initial corpus of each trial with replacement from a larger pool of seeds.
We modify Fuzzbench to allow for each trial to start with a different sampled corpus.


As observed by Boehme et al. \cite{bohme2020expfuzzing}, species discovery is logarithmic over time and test cases.
We sample from the exponential distribution centered at 20\% of the total seed pool for each trial to focus our trials on undersaturated initial coverage levels.

\subsubsection{Seed Origin}

To evaluate the impact of the seed-origin --how the initial corpus was generated-- impacts the performance of fuzzers, we run each fuzzer on seeds generated by prior runs of AFL and libfuzzer and compare the results.
\paragraph{Seed Pools}
To generate the two seed pools used in this experiment, we ran AFL and libfuzzer respectively for 5 repetitions of 24 hours using Fuzzbench's default static seed set.
We then took the final corpora from each of the five repetitions and used aflpp-cmin to reduce these files down to a single pool per origin.
For each trial we sample from the corresponding pool.

\paragraph{Targets} We pick three targets at random from the Fuzzbench benchmarks.
While more targets would be beneficial, running on each target is expensive and we leave further testing to future work.

\paragraph{Repetitions}
We sample from each pool for 24 trials on each benchmark, amounting to ($2 * 24 * 3 = 144$ cpu days of testing time).
We split each benchmark onto a single AWS \textit{c6i.metal} instance using Fuzzbench's local experiment feature to run outside of GCE.


==> nsections/tech1.tex <==



\section{Impact of Individual Properties}\label{sec:first}


%In \autoref{sec:origin}, we saw that different corpus origins are correlated with different benchmarking outcomes.
%In the following section we 
%We investigate how benchmark properties affect absolute and relative fuzzer performance, in terms of branch coverage.
%
%

%
%\subsection{Presentation and Analysis}\vspace{-0.1cm}
%
%
%\paragraph*{Analysis} 
\autoref{fig:effectiveness} illustrates that relationship between benchmark properties affect absolute and relative fuzzer performance, in terms of branch coverage, using  scatter plots of the rank-transformed data.

\autoref{fig:effectiveness}.a plots the \emph{corpus} property of each program-specific trial on the X-axis and the attained coverage of that trial on the Y-axis, both subject to the rank transform per fuzzer-program pair.
The black dots show \emph{average} branch coverage across programs and fuzzers for every level of the corpus property.
The grey dots show the full data for all fuzzers and programs.

\autoref{fig:effectiveness}.b is a similar plot, showing the four \emph{program} properties against the fuzzer performance.
However, %because we are interested in program properties, 
we apply the rank transform w.r.t. all $24 \times 11=264$ trials.
In addition to these two groups of plots in \autoref{fig:effectiveness}, we quantify the direction and strength of these relationships with Spearman's rank correlation ($\rho$) (Fig.~\ref{fig:correlationmatrix}).

Figures~\ref{fig:effectiveness}.c and \ref{fig:effectiveness}.d show the impact of the four measured corpus and program properties, respectively, on the \emph{relative ranking} of each fuzzer.
For example a relative ranking of (1) means that, of the 4 fuzzers we tested, the corresponding fuzzer had the highest edge coverage for that run.
%These plots show how fuzzers may be affected differently by different benchmark properties.
%\vspace{-0.2cm}
\subsection*{RQ.1\quad Impact on Fuzzer Performance}

%\paragraph*{RQ2(A) Results: General Performance} 
Figures~\ref{fig:effectiveness}.a and \ref{fig:effectiveness}.b show the relationship between rank-transformed corpus/program properties and the achieved branch coverage.
For corpus properties, we see a strong ordinal association between the final branch coverage and both the number of seeds as well as the coverage of the initial corpus.
As the starting branch coverage of the initial corpus increases, the final coverage attained also increases.
The average execution time of a seed in the initial corpus and fuzzer performance seems to have a far less pronounced trend, if at all. 

Interestingly, there appears to be a non-linear relationship between the average size of a seed in the initial corpus and the final coverage, resulting in an inverted ``U'' shape.
However, mean seed size alone does not produce this effect.
Further investigation reveals that the corpora in our data set with relatively larger seeds tended to also have fewer such input files.
% This is unsurprising, as we would expect as the sample size of seeds increases the values would tend closer to the mean.
In \autoref{fig:effectiveness}.a, we see that the number of seeds is highly correlated with the final coverage -- thus the nonlinear trend is a result of a \emph{confounding variable}, the corpus size.
While plotting individual explanatory variables against the response can be a useful visualization, one must use a holistic evaluation as described in \autoref{sec:t3} to avoid such issues.

For the program properties, we can see there is a strong positive and linear relationship for the ordinal association between program size and fuzzer performance (cf. Fig.~\ref{fig:effectiveness}.b). %, $\rho=0.74$).
With more code available to be covered, fuzzers are able to reach more code regions in a fixed amount of time.
%Indeed, if regions range in their difficulty to cover, having more regions available in the program means more regions that are more easily reachable, assuming a fixed distribution of difficulty.
For the other properties, from the random scatter and the nearly horizontal regression lines we see no impact.
\vspace{-0.1cm}
\result{For many benchmark properties, there is a \textbf{strong association} between the property and fuzzer performance across all fuzzers.
For instance, fuzzers generally attain higher coverage on larger programs.
We identify the number/size of the seeds, and program size as critical variables to account for during an evaluation. We see no evidence that the quantity of various constraints in real-world programs affects coverage.}%s\vspace{-0.2cm}

%\paragraph*{RQ2(B) Results: Relative Performance}
\subsection*{RQ.2\quad Impact on Fuzzer Ranking}
Figures~\ref{fig:effectiveness}.c and \ref{fig:effectiveness}.d indicate that changes in the individual benchmark properties are associated with changes in the overall rankings of fuzzers at the end of a benchmarking run.
For instance, LibFuzzer's ranking worsens as the coverage, average size and average execution time of the seeds in the seed corpus increases, or as the size of the program increases.
Meanwhile, AFL's ranking improves as coverage and average size of seeds in the initial corpus increases.
Similarly, AFL++'s ranking improves on larger programs or where the initial seed corpus executes faster.
Entropic's ranking appears to be relatively robust to changes in properties of the benchmark.
Note that certain visible trends in \autoref{fig:effectiveness}.c-d are not indicative of statistically significant differences in performance. For example, AFL and LibFuzzer appear to be impacted differently by the number of seeds in \autoref{fig:effectiveness}.a, but their confidence intervals both overlap, i.e., there is no evidence that they behave differently at 95\% confidence level.
We will examine statistically significant effects more closely in the following section.
%
\vspace{-0.1cm}
\result{%
%As program size increases, LibFuzzer's ranking worsens while AFL++'s improves.
Many benchmark properties appear to be correlated with the rank of a fuzzer. For some fuzzers, the ranking is influenced more than for others.
In addition to the {corpus origin} (\autoref{sec:origin}), we found that the {initial coverage}, {number of seeds}, {mean execution time}, {mean seed size} and {program size} are each associated with \textbf{different effects} on disparate fuzzer implementations.}\vspace{-0.1cm}


%\paragraph*{Consequence} In general, the first step in our methodology can be used to visually assess the impact of an \emph{individual} numeric or ordinal benchmark property on a tool or algorithm. Wherever an impact is identified, researchers should ensure that their benchmark is sufficiently diverse w.r.t. these properties. Spearman correlation values also help to quantify the difference between the performance of a fuzzer on the benchmark and the performance of that fuzzer in a specific use case (e.g., given a certain program and initial corpus). However, further steps are needed to assess the combined effects of these variables and avoid confounding influences.

%In addition to the individual fuzzer performance, we are often more concerned with the \emph{relative performance} of two or more tools, like a baseline and a proposed fuzzer. In the following section, we investigate the impact of benchmark properties on benchmarking outcome.



==> nsections/tech2.tex <==

\section{Benchmark Impact on Benchmarking Outcome}
\label{sec:t1}
%\vspace{-0.15cm}
\result{RQ2: What is the impact of a given property of the benchmark \emph{in isolation} on the superiority or ranking of a fuzzer among a set of fuzzers?}\vspace{-0.15cm}

The \emph{benchmarking outcome} is the average ranking across all programs of all fuzzers in terms of their performance. If we only had two fuzzers, we would report the average superiority as outcome.
We compute the ranking of each fuzzer relative to each other fuzzer per trial (i.e. when started on the same initial corpus for the same program).
%Using the current atomistic benchmarking methodology, a practitioner would be guided only by the ranking or superiority of a fuzzer.
By regressing against the ranking of a fuzzer for each trial, we are able to assess the impact of each property on this ranking or superiority.

\textbf{Analysis}. To visually assess the relationship between benchmark property and fuzzer ranking, we propose a simple scatter plot of the ranks but clearly differentiate each fuzzer. Quantitatively, we propose to compute (i)~Spearman's rank correlation ($\rho$) to assess the direction and strength of the relationship, and (ii)~the coefficients of the regression slopes to assess the magnitude of the impact. A large regression slope indicates a large change in ranking. To assess the variance of the regression coefficients, we suggest bootstrapping the coefficient to estimate the 95\%-confidence intervals around the slope coefficient.
%
Figures~\ref{fig:slr}.a and \ref{fig:slr}.b show the impact of the four measured corpus and program properties, respectively, on the ranking of each fuzzer.
\autoref{fig:slr}.c gives the regression coefficients for a linear regression of the ranks of each property value against the ranking of each fuzzer. 


%\textbf{Bootstrap CIs}. To bootstrap 

%\todo{Discuss procedure of non-parametric bootstrap. Discuss BCA.}

\textbf{Results}. As we can see in \autoref{fig:slr} (a) and (b), the individual fuzzer rankings are visibly impacted by the benchmark properties.
For instance, LibFuzzer's ranking worsens as the coverage, average size and average execution time of the seeds in the initial corpus increases, or as the size of the program increases.
Meanwhile, AFL's ranking improves as coverage and average size of seeds in the initial corpus increases.
Similarly, AFL++'s ranking improves on benchmarks with larger programs or where the initial seed corpus executes faster.

% For Entropic, we cannot identify a statistically significant impact of any benchmark property on its ranking.
In \autoref{fig:slr}.c, we consider the effect as statistically significant whenever the 95\%-confidence intervals do not include the origin.
Here we see that some visible trends in \autoref{fig:slr} (a) and (b) are not indicative of statistically significant differences in performance.
For example, AFL and LibFuzzer appear to be impacted differently by the number of seeds in \autoref{fig:slr}.a, but their regression coefficient confidence intervals both overlap zero so we cannot say that they behave differently at the 95\% confidence level.
%For the program properties, we also note that given the small sample size (11 programs), the results should be taken as preliminary.
%\vspace{-0.1cm}

%, e.g., as the coverage of the initial seed corpus increases, the ranking of LibFuzzer worsens while the ranking of AFL appears to improve.
%This leads LibFuzzer to go from being generally ranked above AFL on high-coverage initial corpora to the worst fuzzer on low-coverage initial corpora.
%In \autoref{fig:slr}.c, we see that this flip in rankings between AFL and Libfuzzer corresponds to a significant difference in behavior according to the bootstrapped 95\%-confidence %interval. The impact of initial coverage on the ranking does not seem statistically significant for Entropic and AFL++.
%
%As for the other corpus properties, an increase of the average seed size in the initial corpus worsens the ranking of LibFuzzer but improves that of AFL. An increase of the average execution time also worsens the ranking of LibFuzzer but improves that of AFL++.

%AFL++'s ranking improves with an increase in average execution time or the average size of seeds in the initial corpus while LibFuzzer worsens with an increase in both corpus properties. These differences are statistically significant according to  bootstrapped 95\%-confidence intervals (\autoref{fig:slr}.c).

%For the program properties, we only examine the impact of program size, based on our earlier results presented in \autoref{sec:first}.
%As the size of the  program increases, LibFuzzer  ranks substantially worse while AFL++ starts ranking substantially better. There also seem to be an effect on the ranking of AFL and Entropic, but this effect is not statistically significant according to the bootstrapped 95\%-confidence intervals in \autoref{fig:slr}.c.
%However, we note that given the small sample size (11 programs), the results on the impact of program properties should be taken as preliminary.
\result{%
As program size increases, LibFuzzer's ranking worsens while AFL++'s improves. A ten-rank increase in program size (a difference in ten positions when the programs are sorted from smallest to largest) boosts AFL++'s relative performance by one rank but degrades LibFuzzer's by one rank.
%
LibFuzzer's ranking drastically degrades as any of the measured corpus properties increases.
%
AFL++'s ranking is positively impacted by an increase in execution time or seed size.
%
AFL's ranking is positively impacted by the coverage of  initial corpus.
%
Entropic's ranking is relatively robust to changes in properties of the benchmark. %It does not seem to be affected by benchmark properties, at all.
}


\textbf{Consequence}. The outcome of a fuzzer evaluation (in terms of effect size) \emph{cannot} only be explained by the ground-truth, general, underlying relative performance of each fuzzer. The outcome is also influenced by the specific choice of benchmark. This means, it is insufficient to report only the outcome of an evaluation, as in an atomistic evaluation, even if the specific properties of a benchmark are mentioned. Researchers should also assess the degree to which the specific benchmark properties contribute to the evaluation result.


%\vspace{-0.1cm}


%In summary, single variable regression models against the fuzzer rankings tell us that corpus and benchmark properties are not only correlated with the absolute performance of fuzzers (cf. \autoref{sec:t1}), but with the relative performance as well.
%Practitioners can use this methodology to assess how benchmarking results may be biased with respect to these properties.
%However, without further analysis, we cannot say what the effect of each property is taking into account each of the others.


==> nsections/thresh.tex <==
\subsection*{IRQ5: Threshold Values}

\begin{figure*}
    \centering\footnotesize
    \begin{minipage}{0.45\textwidth}\centering
    \textbf{(a)~Libfuzzer's Ranking Threshold}\\
    \includegraphics[width=\textwidth]{assets/thresh/thresh_heat.png}
    \end{minipage}
    \begin{minipage}{0.3\textwidth}\centering
    \textbf{(b)~Norm. Prop. Values v. Rank Transform }\\
    \includegraphics[width=\textwidth]{assets/thresh/rank_vs_norm.png}
    \end{minipage}
    \caption{(Left) Libfuzzer's predicted ranking heatmap as two properties (execution time and initial coverage) vary. (Right) The normalized concrete values of each property plotted against the rank-transform of that value.\vspace{-0.2cm}}
    \label{fig:thresh}
\end{figure*}

While the rank-transform allows us to make statistically significant claims about the impact of various properties on fuzzer performance, it also introduces a layer of indirection. 
Intuitively, the transformed data is correlated with the underlying concrete values, but the precise relationship may be non-linear or inconsistent, depending on the data itself.
In part, this is because we use the rank transform on data which is not normally distributed or is non-linear.
Indeed, the motivation for utilizing the rank-transform is its agnosticism towards the data, allowing for robust analysis in many scenarios with few assumptions.
However, once significant effects have been detected, it is important to be able to map those results back to the original domain of concrete values.

To illustrate an interpretation of statistically significant effects, we walk through a case study example from (previous section).
There we identified that the initial coverage and execution time both have small, statistically significant effects on the ranking of Libfuzzer.
To visualize these effects, we plot the ranking of Libfuzzer (color) as we vary each variable across the range of possible rank-transformed values in \autoref{fig:thresh} Left.
Cells which correspond to a discrete change of ranking from the top-left minimal value (>0.5 ranking change) are shaded in purple.
Thus the while line between the blue and red cells represents the threshold at which increases in the initial coverage and mean execution time will result in a visible change in the relative ranking of Libfuzzer against other fuzzers.
If instead of using the least coverage, fastest executing corpus, we used the 23rd least coverage, 4th fastest executing corpus, Libfuzzer would do worse relative to other fuzzers. 
The same is true of the 17th least coverage and the 13th fastest corpus, or the 11th and 22nd.
We can also obtain this information directly from the coefficients of the regression model, which predict that Libfuzzer's ranking is a function of $0.03*cov + 0.02*speed$, implying a 16 and 25 rank change would be needed to impact the fuzzer ranking enough to change it in practice (>0.5).

These rank-transformed values, however, still don't give us any information about the concrete values themselves.
At what level of corpus saturation should I stop using Libfuzzer in favor of a different tool?
One can answer this question at varying levels of abstraction.
Our model directly implies that, if you sort the initial corpora for your experiment by saturation (coverage), roughly every 16th corpora will degrade the relative performance of Libfuzzer below the next-best fuzzer.
We can also plot the rank-transformed data against the original values from which it was derived, as in \autoref{fig:thresh} Right.
Here we see that a change of 16 ranks needed to flip Libfuzzers ranking corresponds to about 80\% of the normalized value domain across all benchmarks.
However, for middling ranks, the variance is large, thus 80\% can be seen as an estimate, but not a definitive value.
Going even further, we can look at the concrete values of initial coverage for a single benchmark in isolation (additional figure?).
For the lcms- benchmark, 16 ranks corresponds to about 300 edges of coverage, though again, the exact correspondance is subject to considerable variance.

In summary, we can identify the thresholds needed to change the rankings of various fuzzers and map those thresholds from rank-transformed data to its underlying normalized, or even non-normalized data.
Doing so for the initial coverage of a corpus in our instantiating study, we find that the threshold for Libfuzzer performing worse than the next best fuzzer is crossed after about 16 ranks, or about 80\% of the range of concrete values observed in our experiment.
On the lcms benchmark, this corresponds to around 300 edges.
A similar approach can be used for other variables (or combinations of variables) in a holistic regression model.

==> sections/covariates.tex <==
\section{E2: Covariates and Random Effects}
\include{sections/figures/unfacet-scatters}
Properties of the seed corpus and program under test were collected from the program binaries using objdump and E9patch.

\include{sections/figures/spearman_varclus}

\subsection{Variables Overview}

List the variables, what they are, and how they are acquired.

\subsubsection{Overall Correlations}
Figure \ref{fig:spear-varcorr-e2} shows the variables we measured for each initial corpus and their Spearman correlations with the coverage increase attained for a given run.
From the plot on the left, we can see generally the strength of the effects of these variables across fuzzers and benchmarks.
Here we see that the benchmark itself is among the most important variables that affects the coverage increase.
This indicates that there is a relatively large variance across benchmarks in terms of fuzzer performance.


The plot on the right of Figure \ref{fig:spear-varcorr-e2} clusters variables by their similarity.
Here we see that the initial coverage is likely related to several other variables.

\subsection{Analysis Methodology}

\subsubsection{Proportional Odds Logistic Regression}
\include{sections/figures/po-check}

To see the impact of various covariates on the outcome of benchmarking runs, we look at the relative rank of the fuzzers on each trial.
This approach gives us an ordinal outcome for each fuzzer on each of the 24 trials.
To assess this ordinal data we use Proportional Odds Logistic Regression (POLR).
POLR is an extension of the non-parametric Mann-Whitney U test already widely used in fuzzer benchmarking.
It has the advantages, however, of accounting for the effects of covariates, giving  effect size in the form of the model coefficients and predicting outcomes for unseen data.
The primary requirement of a POLR is the Proportional Odds Assumption.
POLR models, however, can still provide much useful insight when the PO assumption is not met.
Indeed, the Mann-Whitney U test also only has maximum power when the proportional odds assumption is met, yet the assumption is rarely tested.
To check the PO assumption we refer to Figure \ref{fig:po-check}.
Here we see that there are some differences when just looking at each fuzzer across all bencmarks on the left side of the figure.
To examine other variables for the PO assumption, we must stratify them by fuzzer.
The middle plot of Figure \ref{fig:po-check} shows one representative plot for only the AFL fuzzer.
In this plot, we see that, while many of the gaps between points are similarly sized, there are several obvious differences.
However, if we stratify again by benchmark, we see a completely different story.
The right of Figure \ref{fig:po-check} shows an example plot for the AFL fuzzer and HARFBUZZ benchmark.
Here we see clearly uniform gaps between pairs of points.
Unfortunately, this uniformity is not consistent across benchmark and fuzzer pairs.
Additionally, the Brant-Wald test of the Proportional Odds assumption does not hold for the Omnibus test

However, we would like to have some intuition for the impact of these effects across benchmarks to provide general guidance for the fuzzing community.
As a result, coefficients of the model we have fitted across benchmarks should be taken as the net effect across benchmarks, and may not be representative of the effect on a given program.

\subsubsection{Boostrapped Linear Regression}
To assess covariate impact on the coverage increase attained by a given fuzzer, we also use a boostrapped regression model to give a non-parametric linear model.

\subsection{Properties of the Seed Corpus}


\include{sections/figures/e2-polr-table.tex}

\include{sections/figures/e2-polr-coef-plot}

\include{sections/figures/e2-boot-coef-plot}


\subsubsection{Initial Coverage}


Coverage is well known to be discovered at a logarithmic rate over time.
Thus, for a fixed time period such as 24 hours, there is, in essence a "ceiling" of attainable coverage that it is extremely difficult for a fuzzer to break through.
So, any increase in coverage (unless it is not discoverable by a fuzzer at all) ends up causing a reduction in the coverage increase -- there is less new coverage that can be found in the time provided.
The total edges covered, however, does still increase with the initial coverage level.
This happens at lower rate than the additional coverage granted by the seed corpus, and has diminishing returns as the initial corpus coverage approaches the ceiling.

The effect of initial coverage, however, does not appear to be uniform.
Looking at Figure \ref{fig:e2-polr-coef-plot}, we see that relative to the base class of AFL, AFLplusplus is significantly more likely to obtain a better rank as coverage increases (negative coefficient) while libfuzzer and honggfuzz are significantly more likely to obtain a worse rank (positive coefficient).
We can also concretely quantify this effect with the odds-ratio; specifically an odds-ratio of N as in the case of AFL, leads to a X\% chances of improving or degrading the rank of that fuzzer.

\subsubsection{Inequality and Equality Constraints}
\include{assets/ineq-to-initialcover-e2}

The number of inequality and equality constraints exercised by each set of initial seeds per target are remarkably consistent across the benchmarks.
Looking at Figure \ref{fig:ineq-to-init}, we see that the distribution of inequality constraints relative to regions covered by initial seeds is nearly identical across benchmarks.
That is, empirically, programs in Fuzzbench tend to have a similar number of inequality constraints per basic block.
This holds true for equality constraints as well.
Because of this relationship, both metrics correlate very highly with the initial coverage of the seeds of the system under test.


\subsubsection{Corpus Size}

The corpus size is extremely highly correlated with the initial coverage (Spearman correlation for each benchmark $>0.86$).
This high level of correlation is expected, as the corpus was edge-minimized during preprocessing; each test case should correspond to at least one new edge.
As a result, the impact of corpus size is not distinguishable from that of the initial coverage in our experiment.

\subsubsection{Execution Time}
Again, from Figure \ref{fig:ineq-to-init}, we see that libfuzzer is affected negatively by an increase in execution time relative to AFL.
AFLplusplus and Entropic are both likely negatively affected relatively to AFL as well, with confidence intervals only slightly overlapping with zero.
  
\subsubsection{Seed Size}

Seed size has no discernible effect across benchmarks in our experiment, as the confidence intervals are all substantially wider than those for other effects.
Looking at the Spearman correlation of seed size on the coverage increase across benchmarks (\todo{Spearman Corr Figure}, we see that seed side is not well correlated with the coverage increase for many benchmarks.
This likely stems from AFL's file size cap of 1KB, which is enforced across all fuzzers in Fuzzbench.
It seems for these smaller files we cannot say if there is any impact on the overall or relative performance of fuzzers.

\subsection{Program Properties}

\subsubsection{Indirect Jumps, Inequality and Equality Constraints}

\include{sections/figures/static-ind-eq-ineq-scatters}
\include{sections/figures/static-per-line-indir-ineq-eq-scatter}

Figure \ref{fig:static-indir-ineq-eq-scatter} suggests that number of each type of basic block transition statement is positively correlated with the coverage increase attained by fuzzers on that program.
This is likely for similar reasons that the program text size is correlated with coverage increase (or v.v.); more code or transitions in total generally means that there are more dynamically explorable paths for each fuzzer.



However, looking at Figure \ref{fig:static-indir-ineq-eq-scatter-per-e}, we see little to no correlation for the total number of each edge transition type as a ratio of the total transitions.
In other words, the number of inequality constraints per transition in the static program binary has no discernible effect on the coverage increase attainable by fuzzers.
The same appears to be true for equality constraints and indirect jumps.


\subsubsection{Program Size}

\include{sections/figures/static-size-scatter}

Figure \ref{fig:static-size-scatter} shows a relatively stronger positive correlation between the size of the text segment of the binary and the coverage increase.
Intuitively, this is likely because these larger, more complex programs have more code paths that may be explored.
Furthermore, the gaps in performance between fuzzers appears to widen on larger programs.


\subsubsection{Shared Library Calls, }


\include{sections/figures/static-shared-scatter}

While the static number of shared library calls correlates with the size of the program, similarly to the number of inequality constraints or indirect jumps, it appears to differ in its effect on the coverage attained by fuzzers on the target program.

Figure \ref{fig:static-shared-scatter-per-i} shows a negative correlation between the number of shared calls per instruction and the coverage increase.
This could be for a number of reasons -- the calls slow down execution, the shared libraries aren't instrumented.
Symbolic execution engines are known to have difficulty with dynamic libraries, so it is interesting that fuzzers may be similar in this respect.

==> sections/figures/comp-w-fb.tex <==
\begin{figure*}
    \centering
    
    \begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=0.98\textwidth]{assets/compare-w-fb/initial_coverage-3.png}
    \label{fig:cmp-w-fb-ic}
    \end{subfigure}
    
    \begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=0.98\textwidth]{assets/compare-w-fb/mean_size_bytes-3.png}
    \label{fig:cmp-w-fb-msb}
    \end{subfigure}
    
    \begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=0.98\textwidth]{assets/compare-w-fb/mean_exec_ns-3.png}
    \label{fig:cmp-w-fb-mens}
    \end{subfigure}
    
   \caption{Difference in rankings from a reference run of Fuzzbench as initial coverage (top), mean seed size (middle) and mean execution time (bottom) vary across benchmarks}
    \label{fig:cmp-w-fb}
\end{figure*}

==> sections/figures/e1-polr-coef-plot.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{assets/polr-e1/simple_plot.jpg}
    \caption{Selected Coefficients of the POLR Model on per-trial Ranking of Fuzzers for Differing "Seed-Origins"}
    \label{fig:e1-polr-coef-plot}
\end{figure}

==> sections/figures/e1-polr-tabs.tex <==
\begin{figure}\scriptsize
    \begin{minipage}{0.48\columnwidth}\centering
    \textbf{AFL}\\[0.1cm]
    \input{assets/polr-e1/afl}
    \end{minipage}\quad
    \begin{minipage}{0.48\columnwidth}\centering
    \textbf{AFL++}\\[0.1cm]
    \input{assets/polr-e1/aflplusplus}
    \end{minipage}\\[0.3cm]
    \begin{minipage}{0.48\columnwidth}\centering
    \textbf{Entropic}\\[0.1cm]
    \input{assets/polr-e1/entropic}
    \end{minipage}\quad
    \begin{minipage}{0.48\columnwidth}\centering
    \textbf{LibFuzzer}\\[0.1cm]
    \input{assets/polr-e1/libfuzzer}
    \end{minipage} 
    \caption{Selected Corpus Property Regression Tables}
    \label{fig:e2-polr-tabs}
\end{figure}

==> sections/figures/e1-polr.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{ l r r r r }
 \toprule
 Variable &                     Coefficient & S.E.  & Wald Z & Pr($>|Z|$)  \\
 \midrule
corpus=e1v0-libfuzzer &                     -2.8982 & 0.5351 & -5.42 & $<$0.0001 \\
fuzzer=aflplusplus &                         6.9831 & 0.6495 & 10.75 & $<$0.0001 \\
fuzzer=entropic &                            0.6154 & 0.4758 &  1.29 & 0.1959  \\
fuzzer=honggfuzz &                           0.5400 & 0.4969 &  1.09 & 0.2772  \\
fuzzer=libfuzzer &                          -8.4990 & 0.7258 &-11.71 & $<$0.0001 \\
initial\_coverage &                          -0.0019 & 0.0001 &-15.33 & $<$0.0001 \\
corpus=e1v0-libfuzzer * fuzzer=aflplusplus & 2.6883 & 0.7674 &  3.50 & 0.0005  \\
corpus=e1v0-libfuzzer * fuzzer=entropic &    3.3829 & 0.7099 &  4.77 & $<$0.0001 \\
corpus=e1v0-libfuzzer * fuzzer=honggfuzz &   0.9198 & 0.7114 &  1.29 & 0.1960  \\
corpus=e1v0-libfuzzer * fuzzer=libfuzzer &   0.8756 & 0.7007 &  1.25 & 0.2114 \\
 \bottomrule
\end{tabular}
\caption{Coefficients for POLR of sqlite3}
\label{tab:sql-e1-polr}
\end{center}
\end{table*}

\begin{table*}
\begin{center}
\begin{tabular}{ l r r r r }
 \toprule
 Variable &                     Coefficient & S.E.  & Wald Z & Pr($>|Z|$)  \\
 \midrule
corpus=e1v0-libfuzzer   &                    7.0628 & 0.6892 & 10.25 & $<$0.0001 \\
fuzzer=aflplusplus &                         6.4886 & 0.7019 &  9.24 & $<$0.0001 \\
fuzzer=entropic &                            7.3184 & 0.6829 & 10.72 & $<$0.0001 \\
fuzzer=honggfuzz &                           5.8660 & 0.7178 &  8.17 & $<$0.0001 \\
fuzzer=libfuzzer &                           5.6182 & 0.6188 &  9.08 & $<$0.0001 \\
initial\_coverage &                          -0.0123 & 0.0009 &-14.23 & $<$0.0001 \\
corpus=e1v0-libfuzzer * fuzzer=aflplusplus &-5.7830 & 0.7997 & -7.23 & $<$0.0001 \\
corpus=e1v0-libfuzzer * fuzzer=entropic &   -6.9437 & 0.7924 & -8.76 & $<$0.0001 \\
corpus=e1v0-libfuzzer * fuzzer=honggfuzz &  -4.8648 & 0.8109 & -6.00 & $<$0.0001 \\
corpus=e1v0-libfuzzer * fuzzer=libfuzzer &  -7.1324 & 0.8024 & -8.89 & $<$0.0001 \\
 \bottomrule
\end{tabular}
\caption{Coefficients for POLR of lcms}
\label{tab:lcms-e1-polr}
\end{center}
\end{table*}

==> sections/figures/e2-boot-coef-plot.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{assets/e2-logboot-coef-plot.jpg}
    \caption{Selected Coefficients of the Bootstrapped Linear Model on per-trial Ranking of Fuzzers}
    \label{fig:e2-polr-coef-plot}
\end{figure}

==> sections/figures/e2-mr-tabls-vals.tex <==
    \scriptsize
    \begin{minipage}{0.48\columnwidth}\centering
    \textbf{AFL}\\[0.1cm]
    \input{assets/np-boot/afl_mr_val}
    \end{minipage}\quad
    \begin{minipage}{0.48\columnwidth}\centering
    \textbf{AFL++}\\[0.1cm]
    \input{assets/np-boot/aflplusplus_mr_val}
    \end{minipage}\\[0.3cm]
    \begin{minipage}{0.48\columnwidth}\centering
    \textbf{Entropic}\\[0.1cm]
    \input{assets/np-boot/entropic_mr_val}
    \end{minipage}\quad
    \begin{minipage}{0.48\columnwidth}\centering
    \textbf{LibFuzzer}\\[0.1cm]
    \input{assets/np-boot/libfuzzer_mr_val}
    \end{minipage} 



==> sections/figures/e2-mr-tabs.tex <==
\begin{figure}\scriptsize
    \begin{minipage}{0.48\columnwidth}\centering
    \textbf{AFL}\\[0.1cm]
    \input{assets/rank-boot/afl_mr}
    \end{minipage}\quad
    \begin{minipage}{0.48\columnwidth}\centering
    \textbf{AFL++}\\[0.1cm]
    \input{assets/rank-boot/aflplusplus_mr}
    \end{minipage}\\[0.3cm]
    \begin{minipage}{0.48\columnwidth}\centering
    \textbf{Entropic}\\[0.1cm]
    \input{assets/rank-boot/entropic_mr}
    \end{minipage}\quad
    \begin{minipage}{0.48\columnwidth}\centering
    \textbf{LibFuzzer}\\[0.1cm]
    \input{assets/rank-boot/libfuzzer_mr}
    \end{minipage} 
    \caption{Selected Corpus Property Multiple Regression Tables}
    \label{fig:e2-polr-tabs}
\end{figure}

==> sections/figures/e2-polr-tabs.tex <==
\begin{figure}\scriptsize
    \begin{minipage}{0.48\columnwidth}\centering
    \textbf{AFL}\\[0.1cm]
    \input{assets/polr-e2/afl}
    \end{minipage}\quad
    \begin{minipage}{0.48\columnwidth}\centering
    \textbf{AFL++}\\[0.1cm]
    \input{assets/polr-e2/aflplusplus}
    \end{minipage}\\[0.3cm]
    \begin{minipage}{0.48\columnwidth}\centering
    \textbf{Entropic}\\[0.1cm]
    \input{assets/polr-e2/entropic}
    \end{minipage}\quad
    \begin{minipage}{0.48\columnwidth}\centering
    \textbf{LibFuzzer}\\[0.1cm]
    \input{assets/polr-e2/libfuzzer}
    \end{minipage} 
    \caption{Selected Corpus Property Regression Tables, POLR}
    \label{fig:e2-polr-tabs}
\end{figure}

==> sections/figures/e2_mr.tex <==
\begin{figure*}
    \centering
    \include{sections/figures/e2-mr-tabls-vals}
    \begin{minipage}{0.49\textwidth}
    \includegraphics[width=\textwidth]{assets/np-boot/fuzzer-coef.png}
    \label{fig:e2-polr}
    \end{minipage}
    \caption{Selected Coefficients of Multiple Regression Models POLR (left) and MR (right)}
    \label{fig:e2:mr}
\end{figure*}

==> sections/figures/fb-off.tex <==
\begin{figure}
% \centering
\scalebox{0.90}
{
\footnotesize
\begin{minipage}{0.48\columnwidth}
\begin{tabular}{@{}rl}
\multicolumn{2}{@{}l}{\emph{Ranking (5 Smallest Programs)}}\\
Entropic      &        $1.7 \pm 0.84$ \\
AFL++         &        $2.3 \pm 0.97$ \\
LibFuzzer     &        $2.9 \pm 1.14$ \\
AFL           &        $3.1  \pm 1.24$ \\
\end{tabular}\\[0.2cm]
\end{minipage}

\begin{minipage}{0.48\columnwidth}
\begin{tabular}{@{}rl}
\multicolumn{2}{@{}l}{\emph{Ranking (5 Largest Programs)}}\\
AFL++           &      $1.4  \pm 0.55$ \\
AFL             &      $2.2  \pm 0.84$ \\
Entropic        &      $2.4  \pm 0.89$ \\
LibFuzzer       &      $4.0  \pm 0.00$ \\
\end{tabular}\\[0.2cm]
\end{minipage}
}
\end{figure}




==> sections/figures/mr-unified-aflbase-rankvals.tex <==
\begin{figure}\scriptsize
    \input{assets/rank-boot/none_unified_model}
    \caption{Regression Coefficients Against Ranked Edge Coverage}
\end{figure}

==> sections/figures/po-check.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}{0.44\textwidth}
    \includegraphics[width=\textwidth]{assets/e2-po-check.jpg}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
    \includegraphics[width=\textwidth]{assets/e2-po-check-strat-afl.jpg}
    \end{subfigure}

    \caption{Cumulative log-odds to check for PO assumption across all benchmarks and fuzzers (left), for AFL across all benchmarks (right). The spacing between each pair of shapes across rows will be similar when the PO assumption is met.}
    \label{fig:po-check}
\end{figure*}

==> sections/figures/uni-frmr.tex <==
\begin{figure*}[t]
    \centering\footnotesize
    \begin{minipage}{0.18\textwidth}\centering
    %\textbf{(b)~Program properties.}\\
    \includegraphics[width=\textwidth]{assets/uni-rr/big-eff.png}\\
    \scriptsize
    
    $R^2=0.60$, \emph{p-val.}$<0.001$\\
    Median Residuals: $0.042$
    %[0.2cm]\textcolor{white}{.}
    \end{minipage}
    \begin{minipage}{0.81\textwidth}\centering 
    %\textbf{(a)~Corpus properties.}\\
    \includegraphics[width=\textwidth]{assets/uni-rr/small-eff.png}%\\[0.3cm]
    \end{minipage}
    \caption{Multiple Linear Regression with LibFuzzer as reference level (Fuzzer Ranks $\sim$ Fuzzer $\times$ Corpus Properties).}
    \label{fig:mlr}   
\end{figure*} 

==> sections/motivation.tex <==
\section{Motivation}

\include{sections/figures/comp-w-fb}

Covariates and random effects can impact the result of any experimental setup and fuzzing benchmarks are no exception. 
Indeed, prior work \cite{seedsel21} by Herrera et al found that different kinds of initial corpora can have a drastic impact on fuzzer performance.
Equally importantly for fuzzer evaluation, Herrera et al found that these impacts differed across fuzzer implementations.
Such effects, if not accounted for, could lead to misleading benchmarking results.
Potentially compounding the issue, popular fuzzer benchmarks such as Fuzzbench \cite{metzman2021fuzzbench} and Magma \cite{hazimeh2020magma} use a static corpus for each trial; if the starting corpus for a particular is biased with respect to an important covariate, no amount of repetitions will resolve this bias.



Additionally, a benchmarking approach with more nuanced information is useful for both fuzzer developers and users.
For developers, more granular detail about which factors lead to poor or good performance can lead to improvements in fuzzer implementations.
For users, information about which fuzzers perform best in which contexts allows them to pick the best fuzzer for their own systems.

Various aspects of the seed corpus and program under test are widely thought or known to have an impact on Fuzzer performance.
For example, AFL rejects seeds that are too large or too slow by default.
Finding appropriate seeds is difficult, and it would be impossible to change one aspect of the seed corpus while holding all others constant.
Thus the current pairwise statistical tests preferred by fuzzer evaluators pairwise are insufficient to rigorously determine the impact of such changes in the initial corpus or otherwise.

==> sections/seed-origin.tex <==
\section{E1: Seed Origin}
\todo{Might be better to organize the result sections around the research questions instead of the experiments. Seed origin is only one bullet point under RQ1. You could move setup to \autoref{sec:setup}.}


\subsection{Results}
\input{sections/figures/e1violin}

\input{sections/figures/tiny-e1-ahat}

 We summarize the results of this experiment in Figure \ref{fig:e1-viol} and \ref{fig:seedorigin-ahat}.
 The former shows violin plots of each fuzzer's performance on the various benchmarks with each corpus.
 The latter shows Fuzzbench's reports of significance and effect size for the LCMS program.
 
 Visual inspection of the violin plots on the left and right sides of Figure \ref{fig:e1-viol} are relatively similar.
 However, especially for AFL and libfuzzer, there are significant differences in coverage on the difference corpora.
 For example, while AFL is clearly the worst performer on the AFL-seeded corpus on the lcms benchmark, it is comparable in performace to the others on the libfuzzer-seeded corpus.
 Indeed, looking at the p-values and effect size reported in Figure \ref{fig:seedorigin-ahat}, we see that all other fuzzers significantly outperform AFL on the AFL-seeded corpus and all other fuzzers significantly outperform libfuzzer on the libfuzzer-seeded corpus.
 This difference is expected; if there are regions found only by AFL on a particular benchmark, by including testcases that cover those regions we give an advantage to non-AFL fuzzers.
 Indeed, we see no difference across the corpora for the ZLIB benchmark, where there are no completely unique regions for any of the tested fuzzers.
 
 
 Additionally, while not obvious from the violin plots, this seems to carry over to derivative fuzzers in some cases as well.
 Entropic, a libfuzzer derivative, performs moderately better than honggfuzz (VDA of 0.63, $p < 0.5$) on the AFL seeded corpus, but performs much worse than honggfuzz on the libfuzzer-seeded corpus (VDA of 0.27. $p < 0.01$).
 This change suggests that derivatives of fuzzers can also be impacted if the initial corpus was generated by it's base fuzzer.
 
 \todo{Reorganize a bit: bring some conclusions and data to beginning. Something like: "The fuzzer that generated the seed corpus (and its derivatives) is X times less likely to outperform a fuzzer that did not generate the seed corpus".}

\iffalse
 \subsection{Possible Confounding Variables}
\todo{As this is only an auxiliary investigation, this section and the corresponding tables might go into the appendix. We also need instructions on how to interpret the tables and related terms.}
We examined other characteristics of the two initial corpora to ensure that these other random effects are not confounding for the seed origin.
For example, on the LCMS target, the distribution of initial coverages between the AFL-seeded and libfuzzer-seeded corpora is notably different.
Additionally, for the SQLITE3 target, the distribution of mean seed sizes is drastically different.
If either of these variables strongly influences fuzzer performance, we could be misinterpreting the results of this experiment.
To control for these effects, we create a regression model of the form:

$$coverage\_inc ~ corpus + fuzzer + initial\_coverage$$
$$mean\_seed\_size + corpus*fuzzer$$

In this model, we see that the seed size has little to no impact on the model, eliminating it as a possible confounder.
Removing it from the model, we are left with the coefficients shown in Tables \ref{tab:lcms-e1-polr} and \ref{tab:sql-e1-polr}.
Here we see that there are large differences in the coefficients for the interaction terms of the corpus origin and the fuzzer.
In other words, different fuzzers are impacted by the corpus origin differently, even taking into account differences in initial coverage and seed size.
This is significant as seeds are often drawn from prior fuzzing runs in fuzzing evaluation and in practice.
 
\input{sections/figures/e1-polr}
\fi
